Revealing CNN Architectures via Side-Channel Analysis in Dataflow-based Inference Accelerators

Convolutional Neural Networks (CNNs) are widely used in various domains, including image recognition, medical diagnosis and autonomous driving. Recent advances in dataflow-based CNN accelerators have enabled CNN inference in resource-constrained edge devices. These dataflow accelerators utilize inherent data reuse of convolution layers to process CNN models efficiently. Concealing the architecture of CNN models is critical for privacy and security. This article evaluates memory-based side-channel information to recover CNN architectures from dataflow-based CNN inference accelerators. The proposed attack exploits spatial and temporal data reuse of the dataflow mapping on CNN accelerators and architectural hints to recover the structure of CNN models. Experimental results demonstrate that our proposed side-channel attack can recover the structures of popular CNN models, namely, Lenet, Alexnet, VGGnet16, and YOLOv2.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/comments.tex <==
\newpage

\section{Responses to Reviewer Comments}
We would like to thank the reviewers for their thorough and insightful comments. We have modified the manuscript to address various issues raised by the reviewers. This section outlines all the reviewer comments and our responses in terms of how we have addressed the issues in the modified manuscript. The modifications are marked in blue in the manuscript. 

\vspace{0.05in}
\subsection{REVIEWER 1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent \textbf{Comment 1:} Does the method scale for more complex and larger architecture, and especially on custom tailored model?

\color{blue}

\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. Our method inherently scales for more complex and larger architectures.  It employs a layer-by-layer extraction technique, ensuring that the number of layers in a CNN, regardless of depth, does not impede the scalability of our architecture recovery mechanism.  If we consider recovery of parameters in one layer, the core of the method relies on the integer factorization of side-channel information related to number of weight, output, and input reads and writes. 
%Given the advancements in current computational capabilities, it is well-established that factorizing a 512-bit number, approximately equivalent to 154 decimal digits, is feasible. 
Typical side-channel information values for our attacks are around 10 decimal digits, which are well within the range of current computational factorization capabilities. Therefore, our method is scalable for larger and complex architectures. We have successfully applied our attack to custom-tailored models, such as YOLOv2~\cite{redmon2016you}, which is used for object detection and deviates from traditional CNNs by not having fully connected layers. YOLOv2 have 23 convolution layers with 3x3 and 1x1 filters, and 5 max pooling layers with filter size and stride of 2. We are able to recover its architecture across all tested weight stationary (WS) and output stationary (OS) dataflow accelerator configurations, as shown in Table~\ref{tab:com-final-results}. We have updated Table~\ref{tab:final-results} with new results and made corresponding revisions to Section~\ref{sec:experiments}, detailing new experiments and discussing the scalability of our method.

\begin{table}[htp]
\centering
\caption{\textcolor{blue}{Number of potential structures recovered from Lenet, Alexnet, VGGnet-16 and YOLOv2 using our method and comparison with ~\cite{hua2018reverse} that exploit DRAM to GB memory access on temporal inference accelerator.}}
% \vspace{-0.1in}
\resizebox{0.60\textwidth}{!}{%
\begin{tabular}{|ll|l|c|c|c|}
\hline
\multicolumn{2}{|l|}{\textbf{CNN model}} & \textbf{Lenet} & \textbf{Alexnet} & \textbf{VGGnet-16} & \multicolumn{1}{l|}{\textbf{YOLOv2}} \\ \hline
\multicolumn{2}{|l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Number of layers\\ (Conv/Pool/FC)\end{tabular}}} & 3/2/2 & 5/3/3 & 13/5/3 & 23/5/0 \\ \hline
\multicolumn{2}{|l|}{\textbf{Conv layer filter sizes}} & \begin{tabular}[c]{@{}l@{}}5x5\\ 2x2\end{tabular} & \begin{tabular}[c]{@{}c@{}}11x11\\ 5x5, 3x3\end{tabular} & \begin{tabular}[c]{@{}c@{}}1x1\\ 3x3\end{tabular} & \begin{tabular}[c]{@{}c@{}}1x1\\ 3x3\end{tabular} \\ \hline
\multicolumn{1}{|l|}{\multirow{7}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Number of \\ potential\\ structures\end{tabular}}}} & \textit{WS(4,4)} & 1 & 1 & 1 & 1 \\ \cline{2-6} 
\multicolumn{1}{|l|}{} & \textit{WS(12,4)} & 1 & 1 & 1 & 1 \\ \cline{2-6} 
\multicolumn{1}{|l|}{} & \textit{WS(24,10)} & 1 & 1 & 1 & 1 \\ \cline{2-6} 
\multicolumn{1}{|l|}{} & \textit{OS(4,4)} & 1 & 1 & 1 & 1 \\ \cline{2-6} 
\multicolumn{1}{|l|}{} & \textit{OS(10,4)} & 1 & 1 & 1 & 1 \\ \cline{2-6} 
\multicolumn{1}{|l|}{} & \textit{OS(20,10)} & 1 & 1 & 1 & 1 \\ \cline{2-6} 
\multicolumn{1}{|l|}{} & \cite{hua2018reverse} & 9 & 24 & - & - \\ \hline
\end{tabular}%%
}
\label{tab:com-final-results}
% \vspace{-0.10in}
\end{table}

% \begin{itemize}
%     \item Yes, it scales for more complex and larger architectures. Since the proposed model extraction focus on layer by layer extraction of the layer structures the depth of the CNN model (number of layers) does not limit the scalability of our CNN architecture extraction mechanism. 
%     \item If we consider recovering of parameters in one layer that depend on integer factorization of number of weight/output/input reads and writes (side channel information). With current computational power it is well known that factorization of 512-bit number ($\approx$ 154 decimal digits) is possible. This is well over the any  side channel value which is around 10 decimal digits. Therefore, our method is scalable for larger and complex architectures.
%     \item We conducted our attack on two other custom tailored model YOLOv2~\cite{redmon2016you} that used for object detection when using all WS and OS dataflow accelerator configurations used in Table~\ref{tab:final-results}.
%     \item YOLOv2 is different from traditional CNN because it doe not have fully connected layers. YOLOv2 has 23 convolution layers with filter size of 3x3 and 1x1 and 5 max pooling layers with filter size 2 and stride 2.
%     \item we were able to recover the YOLOv2 architecture from all all WS and OS dataflow accelerator configurations
% \end{itemize}

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 2:} Since the proposed method recovers the architecture, what are potential threat for the model owner?

\color{blue}

\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. The recovery of a CNN model’s architecture poses significant risks for the model owner. (1) If the structure of a CNN is disclosed, it becomes easier for adversaries to craft efficient adversarial attacks~\cite{chakraborty2018adversarial, hu2020deepsniffer} fine-tuned to mislead the model without detection, thereby facilitating evasion attacks. For example, if a particular model is used to detect and flag network anomalies, an adversary can manipulate network traffic in such a way that it evades detection, allowing malicious activities to proceed undetected and model owner failing to provide the intended functionality. (2) The exposure of the model architecture can lead to the leakage of proprietary and critical intellectual property. For many companies, the design of their models embodies valuable research and development efforts, and unauthorized access to this information can lead to competitive disadvantages and economic losses. (3) As outlined in our paper, the leakage of model architecture in environments where the hardware is shared, increases the risk of user privacy breaches. Adversaries can exploit the known architecture to perform more effective model inversion attacks~\cite{fredrikson2015model}, potentially reconstructing sensitive training data. In summary, there are various potential threats from the recovery of a models’s architecture, including feasibility of adversarial attacks, loss of intellectual property, and breaches of user privacy, all of which can have severe consequences for the model owner. We have included this discussion at end of Section~\ref{subsec:threat_model_details} to highlight broader implications of proposed attack.


% the model is an intelectual property, so the architture acan be leaked and use for counterfit models. futhermore adversaries can craft better adverserial examples after recovering the model which will lead to evasion in detection bith for model owner and user

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 3:} Regarding the identification of layer boundary, the paper states the adversary could use snooping or hardware Trojan. How feasible are these approaches in practical setting?

\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. Bus snooping is a low-cost, practical and well understood attack that has been widely demonstrated~\cite{huang2002keeping,huang2014hmtt,blass2012tresor}. Our study utilizes two extraction methods for side-channel information: snooping via Hardware Trojans (HT) and microprobing. These methods are well-studied threat models for DNN extraction in GPUs and other temporal DNN accelerators~\cite{hua2018reverse, hu2020deepsniffer}. We briefly describe them and outline their feasibility. We have included this discussion in Section~\ref{subsec:threat_model_details}. 

\noindent
\textit{\underline{Hardware Trojans (HT)}}: These accelerators are part of larger System-on-Chip (SoC) designs. SoCs frequently utilize third-party IPs to reduce design and verification cost. For instance, the FlexNoc interconnect  facilitates on-chip communication used by four of the top five fabless companies~\cite{weerasena2023security}. However, this reliance on a long, distributed, and potentially untrusted supply chain raises the risk of malicious implants, such as HTs, introduced through various channels including untrusted CAD tools, rogue designers, or directly at the foundry \cite{mishra2017hardware}. The specific functionality of the HT used in layer identification of our proposed attack is relatively straightforward, comprising merely a comparator that compare two addresses. Similarly, the other HT used for side channel information leak have a counter to track number of memory reads and writes. Such HTs are characterized by their minimal area and power overhead, which helps them to be undetected both in post-silicon testing and runtime monitoring~\cite{ahmed2020defense}. Therefore, it is feasible to use HTs to extract side-channel information from datflow-based accelerators. We have also performed experiments (Section~\ref{sec:experiments}) to deploy hardware Trojans in FPGA-implemented dataflow-based accelerators and recover CNN model architectures.

\noindent
\textit{\underline{Microprobing}}: This technique involves directly accessing internal wires of a hardware module to extract sensitive information. Advances in technology have enhanced microprobing capabilities, allowing for the extraction of data from complicated and thoroughly packed hardware implementations. These probing techniques have been used successfully to extract encryption keys, code format intellectual property, and personal data~\cite{shi2016layout}. For example, state-of-the-art optical probing techniques have been used to steal FPGA bitstream decryption keys from 28nm Xilinx devices~\cite{tajik2017power}. Furthermore, focused ion beam based microprobing has been effective in SoCs to extract information from buses~\cite{wang2017probing}. These methods highlight that precise extraction of data from buses, similar to addresses needed for layer boundary identification, is feasible.


% \begin{itemize}
%     \item Divide answer into snooping and HT
%     \item HT can be insert into netlist... bla bla bla
%     \item since its a simple counter their are and power overhead is negligible 
%     \item can use the same RTL and calcultae area power overhead and see
%     \item \textbf{Snooping}
%     \item microprobing examples and it can detect the 
% \end{itemize}


% -----

% \begin{itemize}
%     \item Snooping bus give example and see that those level of snooping is possible.
%     \item HT is a simple coutnter with a negligible overhead (area, power performance) so harder to detect, explain the concept of RTHT. Give examples for such small HT and how it's hard to detect.
%     \item We conduct WS on a FPGA and 
%     \item Our comparison paper also have talk about snooping and similar threat model.
% \end{itemize}

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 4:} With regards to the attack, what countermeasures that can be proposed to mitigate the potential threat?


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. While this paper primarily focuses on demonstrating the attack, we recognize the importance of discussing potential countermeasures to assist designers in securing CNN architectures. Several mitigation strategies can be explored by the designers. (1) Introducing dummy operations that do not affect the final output but alter the memory access patterns and computational behavior can help obscure the true operations being executed, thereby confusing attackers and complicating their analysis of side-channel data. (2) Implementing variable precision for weights and activations can make it more challenging for attackers to determine the number of memory reads and writes, increasing the difficulty of correlating observed memory operations with specific network layer structures. (3) Employing decoy architectures and alternative data paths that activate during specific operations can mislead attackers about the actual computational processes. (4) Specifically for output stationary (OS) dataflow architectures, randomizing the order of data storage in memory, such as weights and activations, can prevent attackers from easily correlating observed memory access patterns with specific operations. These countermeasures can also be combined to form a multi-layered defense strategy against side-channel attacks. We have included this discussion in Section~\ref{subsec:potential_mitigation_techniques} as potential mitigation techniques.



% Thank you for your comment and suggestion. This paper focuses on attack only. We believe designers can explore various countermeasures as discussed below. Add dummy operations that do not affect the final output but alter the memory access patterns (number of memory reads and writes) and computational behavior to confuse the attacker send the adversary off the calculations. Designers can incorporate variable precision computing through variable precision of weights and activations which will make it harder for the attacker to recover number of memory reads and writes as side channel information. Introduce alternative data paths and decoy architectures that are activated during certain operations to mislead attackers. Specifically for OS dataflow randomize the order of data storage in memory, such as weights and activations, to prevent attackers from easily correlating observed memory access patterns. 

\color{black}
\vspace{0.1in}
\subsection{REVIEWER 2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent \textbf{Comment 1:} Why do authors consider those three architectures? While I agree they have "historical" relevance, I doubt that Lenet and AlexNet to be used in practice much. Or could the authors provide some examples where they are used?

\color{blue}

\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. The selection of the Lenet and AlexNet architectures for our study, despite their lesser utilization in contemporary applications, was primarily their common use as benchmarks in related research in extracting CNN architectures~\cite{hua2018reverse}. This allows for a direct comparison with previous work, ensuring that our results are comparable and that improvements or differences can be systematically assessed. Despite their relative simplicity, architectures such as LeNet and AlexNet are foundational and used as benchmarks in state-of-the-art dataflow-based inference accelerators~\cite{chen2019eyeriss,kwon2018maeri,du2015shidiannao} because they incorporate filter sizes and structural patterns that are common in more complex models today. By successfully conducting layer-by-layer extraction on these architectures, we demonstrate the general efficacy of our attack. In the revised version, we have also incorporated results from YOLOv2~\cite{redmon2016you}, further highlighting the versatility and applicability of our approach across diverse architectures. We have included this discussion and results for YOLOv2 in Section~\ref{sec:experiments}.


% \begin{itemize}
%     \item benchmarks and comparison with previous work
%     \item we also considered custom models as discussed in previous
%     \item Eventhough they are not used frequently they have filter sizes that used in most frequently used models.
% \end{itemize}

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 2:} "(3) User privacy can be compromised in a shared accelerator if the model type is leaked."  -> how?

\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. The term "model type" has been changed to "model architecture" to enhance clarity in our discussion. In shared computing environments with accelerators, different users may deploy their models on the same hardware resources. If the architecture of a particular CNN model is leaked, it could reveal specific data processing characteristics or intended uses that are unique to that model. For example, a model designed for facial recognition or personal data such as medical data analysis could imply that sensitive personal data is being processed. Furthermore, the knowledge of the model's architecture could assist in model inversion attacks~\cite{fredrikson2015model}. Model inversion attacks involve reconstructing the training data of a neural network by exploiting knowledge of the model’s architecture, thereby revealing sensitive information. For example, adversary can recover training data used for a facial recognition/analysis model, compromising privacy of the subjects of the training data. We have rephrased the sentence and expanded the explanation in Section~\ref{sec:introduction} to include these details.



\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 3:} "Due to the inherent difference in computing paradigm and underlying architecture, existing side-channel attacks on GPU/CPU based
accelerators cannot be directly applied to dataflow-based accelerators."  -> please discuss more as it is not clear why ?


\begin{figure}[htp]
% \vspace{-0.15in}
\includegraphics[width=0.6\textwidth]{../figures/temporal_vs_spatial.png}
\vspace{-0.2in}
\caption{Temporal vs Spatial architectures for CNN inference~\cite{sze2017efficient}.}
\label{fig:spatial_vs_temporal}
% \vspace{-0.20in}
\end{figure}

\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. As shown in Figure~\ref{fig:spatial_vs_temporal}, the architectures of CNN inference accelerators can be classified into two paradigms: temporal and spatial~\cite{sze2017efficient}. CPUs and GPUs are considered temporal architectures while dataflow architectures are considered spatial. Temporal architectures enhance parallelism through vectors (SIMD) or parallel threads (SIMT), and maintain a centralized control over numerous Arithmetic Logic Units (ALUs). These ALUs are restricted to fetching data from the memory hierarchy without direct inter-ALU communication. They map both fully connected (FC) and convolutional (CONV) layers to matrix multiplications for parallelized MAC operations. For instance, the convolution operation can be reformulated as matrix multiplication by converting one of the inputs into a Toeplitz matrix~\cite{strang1986proposal}, which is used in temporal accelerators. In spatial (dataflow) architecture, each ALU is equipped with its own control logic and local memory. An ALU with its own local memory is referred to as a processing element (PE). These PEs form a processing chain allowing direct data transfer between them. These architectures do not necessitate mapping FC and CONV layers to generic matrix operations, enabling a more natural execution of DNN layers via individual MAC operations. Dataflow accelerators mitigate the memory bottlenecks common in temporal architectures by introducing multiple levels of local memory hierarchy and interconnects. These include global buffers connecting to DRAM, small local registers within each PE, and an inter-PE network facilitating direct data transfers between PEs. This memory structure significantly boosts energy efficiency by reducing the cost of data accesses by fetching data from local registers or neighboring PEs consuming substantially less energy than accessing DRAM~\cite{sze2017efficient}. 

Due to the differences in architecture and processing mechanism between the two paradigms, existing attacks designed for model extraction on CPUs/GPUs cannot be directly applied to dataflow architectures. If we focus on the proposed attack, the raw side-channel features used in the attack is the number of weights, input reads and partial sum/output reads and writes. If we consider number of input reads ($I_r$) of a CONV layer on a GPU, it reflects the matrix sizes in matrix multiplication representation of CONV layer. Here, there will be duplicate input reads from the memory subsystem where number of duplicate reads reflect the number of filters in that layer. If we analyze a dataflow-based inference accelerator and collect $I_r$, the results will depend on the input forwarding mechanism within the accelerator and the type of data that remains stationary at each PE. Consequently, to recover the model structure from temporal CNN inference accelerators using number of memory reads as side-channels, microarchitectural insights and distinct mechanisms are required to recover model from side-channel data, as opposed to those used for spatial architectures. Furthermore, due to the difference in architecture and data movement, any other side channel (timing, power, and kernal) would be significantly different between temporal and spatial paradigms. Thus any mechanism used in CPU/GPU cannot be directly applied in novel dataflow accelerators. We have added this discussion to Section~\ref{sec:background}, highlighting the inherent differences between the two computing paradigms and explaining why attacks on CPUs/GPUs are not applicable to dataflow architectures.  

\color{black}

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 4:} Please provide a more clear comparison with related work (especially~\cite{hua2018reverse}) and discussion on the contributions of this work.

% TODO explicitly say ....

\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. All the related works of model extraction attacks, including~\cite{hua2018reverse}, are conducted on temporal architectures. Our proposed attack targets spatial (dataflow) architectures to recover CNN structures. As discussed in Comment 3, due to inherent differences in architecture and processing mechanism side-channel attacks on temporal architectures cannot be directly applied to dataflow-based inference accelerators. Specifically, Hua et al.~\cite{hua2018reverse} conducted the attack on a temporal CNN accelerator that facilitates matrix multiplication for DNNs. They utilize side-channel information as number of memory accesses of each data type (weight, activations, partial sums), memory address patterns, access frequencies, and execution times to deduce DNN architectures. Our attack also utilizes the number of memory accesses of each type, similar to~\cite{hua2018reverse}, but does not rely on other side-channel information. Instead, we incorporate architectural hints with side-channel information and propose a novel mechanism tailored for dataflow architectures to recover CNN model structures. This detailed comparative analysis has been added to Section~\ref{subsec:related_work}.



% Thank you for your comment. In Section~\ref{subsec:related_work}, we discuss related works, including ~\cite{hua2018reverse}, which primarily investigates model extraction attacks on temporal architectures within CNN accelerators. These studies, including the one by Hua et al.~\cite{hua2018reverse}, typically analyze FPGA implementation of an CNN accelerator that facilitate matrix multiplication in DNNs, employing metrics like memory addresses, access frequencies, and execution times to deduce architectural details. In contrast, our work focuses on spatial (dataflow) architectures, employing a novel approach that leverages both the count of memory accesses and microarchitectural cues to reconstruct the CNN structure from dataflow-based inference accelerators. This emphasis not only differentiates our research but also explores a less-studied area that could yield insights into the security vulnerabilities specific to dataflow architectures. Furthermore, we contribute to the body of knowledge by detailing how these microarchitectural elements influence the effectiveness of model extraction attacks and potentially offer different security challenges compared to temporal architectures. This detailed comparative analysis has been added to Section~\ref{subsec:related_work}.

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 5:} The same relationship holds for $Y$ and $Y'$. -> $Y$ and $Y'$ are not defined.


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. $Y$ and $Y'$ are input feature map (ifmap) height and output feature map (ofmap) height, respectively. They are defined in the legend box of Figure~\ref{fig:computation_in_cnn}. 


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 6:} Our study focuses on the dataflow aspect of the accelerator by using a generic WS (Section 2.2.1) and OS (Section 2.2.2) -> why?

\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. While there are several types of dataflows, including weight stationary (WS), output stationary (OS), input stationary (IS), and row stationary (RS), this paper focuses on two most widely used configurations~\cite{sze2017efficient}: WS (Section 2.2.1) and OS (Section 2.2.2). Section~\ref{subsec:applicability} outlines how to extend the proposed attacks for other types of dataflows. Given the variability in designs of existing WS and OS dataflow accelerators, including differences in the number of processing arrays and processing elements per array, we use a symbolic representation for generic WS and OS architectures to discuss the attack in Section~\ref{sec:methodalogy}. This approach enhances the generalizability and adaptability of our findings across wide range of accelerators. In Section~\ref{sec:experiments}, we apply these methodologies to specific accelerator models to validate the effectiveness of our proposed attack, demonstrating its relevance across different configurations. We have included this explanation in Section~\ref{subsec:dataflow-based DNN accelerators}.


% Thank you for your comment. Our attack specifically targets the dataflow characteristics inherent in Weight Stationary (WS) and Output Stationary (OS) paradigms, which are pivotal to how data is processed within accelerators. Given the variability in designs of existing dataflow accelerators, such as differences in the number of processing arrays and processing elements per array, we have adopted a symbolic representation of accelerator architecture to discuss attack in Section~\ref{sec:methodalogy}. This generic representation allows our discussion to be broadly applicable across various WS and OS dataflow accelerators, enhancing the generalizability and adaptability of our findings. Subsequently, in Section~\ref{sec:experiments}, we apply these generic methodologies to specific accelerator models to validate the effectiveness of our proposed attack in practical scenarios, demonstrating its applicability and relevance to different accelerator configurations.


% \begin{itemize}
%     \item Our attack exploit the dataflow of the accelerator (either WS or OS).
%     \item Since there are different compositions of the dataflow accelerators with subtle changes (e.g. no of processing arrays, no of processing elements per array)
%     \item we use the generic representation (symbolic representation) of the accelerator architecture to discuss the attack in section~\ref{sec:methodalogy} make the attack more generic across all WS and OS dataflow accelerators and use concrete accelerators to evaluate the proposed attack on  section ~\ref{sec:experiments}.
% \end{itemize}

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 7:} Section 2 provides a lot of information but I find it somewhat inaccessible without prior knowledge. Maybe the authors could improve this section to be a better fit for wider audience.


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your feedback. To improve readability, we made two major changes: First, we added a paragraph at the beginning to introduce deep neural networks (DNNs) and explain fundamental terms related to DNNs. This introduction is designed to prepare readers for the subsequent, more detailed discussions on convolutional neural networks (CNNs) and convolution layers. Second, we created a new subsection titled `Architectures for CNN inference', which discusses the inference process and distinguishes the two architectural paradigms (spatial and temporal) used in CNN inference accelerators. 
%This addition aids readers in gaining a deeper understanding of the following discussions surrounding dataflow-based inference accelerators.



% Thank you for your comment. Addressing your comment we have refine and improve the Section~\ref{sec:background} to address wider audience. We have done two major changes and refine the whole section. 1. We have added a paragraph to introduce and describe terms in deep neural networks (DNNs) before dive into CNNs and convolution layers. Then we have added separate subsection (Architectures for CNN inference), which discuss the inference process and define and explain two architural pardigms : spatial and temporal for CNN infernce accelerators. 

% \begin{itemize}
%     \item provide more detail on dataflow paradigm from the eyeris slides and make the flow more smooth.
% \end{itemize}

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 8:} I find threat model section to be a bit unclear. Please separate into subsections problem definition and threat model.

\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your suggestion. We have divided the section into two subsections as problem formulation and threat model.


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 9:} The authors mention snooping, but do not discuss how realistic is to do it. Similar for microprobing of buses or lightweight HT insertion.


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. Bus snooping is a low-cost, practical and well understood attack that has been widely demonstrated~\cite{huang2002keeping,huang2014hmtt,blass2012tresor}. Our study utilizes two extraction methods for side-channel information: snooping via Hardware Trojans (HT) and microprobing. These methods are well-studied threat models for DNN extraction in GPUs and other temporal DNN accelerators~\cite{hua2018reverse, hu2020deepsniffer}. We briefly describe them and outline their feasibility. We have included this discussion in Section~\ref{subsec:threat_model_details}. 

\noindent
\textit{\underline{Hardware Trojans (HT)}}: These accelerators are part of larger System-on-Chip (SoC) designs. SoCs frequently utilize third-party IPs to reduce design and verification cost. For instance, the FlexNoc interconnect  facilitates on-chip communication used by four of the top five fabless companies~\cite{weerasena2023security}. However, this reliance on a long, distributed, and potentially untrusted supply chain raises the risk of malicious implants, such as HTs, introduced through various channels including untrusted CAD tools, rogue designers, or directly at the foundry \cite{mishra2017hardware}. The specific functionality of the HT used in our proposed attack is relatively straightforward, comprising merely a counter to track number of memory reads and writes. Such HTs are characterized by their minimal area and power overhead, which helps them to be undetected both in post-silicon testing and runtime monitoring~\cite{ahmed2020defense}. Therefore, it is feasible to use HTs to extract side-channel information from datflow-based accelerators. We have also performed experiments (Section~\ref{sec:experiments}) to deploy hardware Trojans in FPGA-implemented dataflow-based accelerators and recover CNN model architectures.

\noindent
\textit{\underline{Microprobing}}: This technique involves directly accessing internal wires of a hardware module to extract sensitive information. Advances in technology have enhanced microprobing capabilities, allowing for the extraction of data from complicated and thoroughly packed hardware implementations. These probing techniques have been used successfully to extract encryption keys, code format intellectual property, and personal data~\cite{shi2016layout}. For example, state-of-the-art optical probing techniques have been used to steal FPGA bitstream decryption keys from 28nm Xilinx devices~\cite{tajik2017power}. Furthermore, focused ion beam based microprobing has been effective in SoCs to extract information from buses~\cite{wang2017probing}. These methods highlight that precise extraction of data from buses, similar to data access counts necessary for our attack, is feasible.

% \begin{itemize}
%     \item We provide two ways to extract side channel information via snooping : via HT and microprobing
%     \item These accelerator will be included a part of a larger System on chip (SoC). SoC development relies on third-party IPs to cut costs and meet market deadlines. For example, FlexNoc interconnect is used by four out of the top five fabless companies to facilitate their on-chip communication \cite{weerasena2023security}. This long, distributed potentially untrusted supply chain can lead to the introduction of malicious implants such as HTs through various avenues, such as untrusted  CAD  tools, rogue designers, or at the foundry~\cite{mishra2017hardware}.
%     \item If we focus on the functionality of the HT needed for the proposed attack, it is a simple HT with a counter and such HTs have small area and power overhead making the detection of HT challenging~\cite{ahmed2020defense}.
%     \item Microprobing directly accesses
%     the internal wires of a module and
%     extracts sensitive information. They have been improved over the years with technology advancement. These probing techniques have been used successfully to extract encryption keys, code format intellectual property and personal data~\cite{shi2016layout}. For example, State-of-the-art optical probing techniques have also been demonstrated to steal on-chip FPGA bitstream decryption keys on 28 nm Xilinx devices~\cite{tajik2017power}. Furthermore, focused ion beam based microprobing have been used as the most powerful for microprobing in lower dimensional SoCs~\cite{wang2017probing}. 
%     \item In our attack we only need the count of data access and successful and precise extraction of more granular data as encryption keys are proof that extracting accurate data access count is possible.
%     \item 
%     \item similar threat models of using HT and microprobing has been used to extract models in GPUs and other temporal CNN accelerators~\cite{hua2018reverse, hu2020deepsniffer}. 
%     \item We have included this discussion on Section~\ref{subsec:threat_model}.
%     \item For the request of reviewer 3 we have provided experimental results on using HT to recover CNN model architecture. 
% \end{itemize}


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 10:} It is important to notice that if there are multiple potential structures for the previous layer, the algorithm tries ifmap parameters ($X, Y, C$) of all of them to recover -> please discuss more as it is not clear how much of a limitation this is. I could imagine that in general, there could be many architectures? Also, what happens when there are minor changes between architectures? The technique is not 100\%? So, can it happen that we recover a similar structure?


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. Our method employs a layer-by-layer structure extraction mechanism. The core of the mechanism for extraction of layer structure involves integer factorization to establish an initial set of potential results and then filtering them through a set of rules informed by architectural hints and side-channel information to converge on a singular structure for a layer. Experimental results across 64 layers in all CNN models tested on six different dataflow accelerators (384 combinations) consistently converged to a single layer structure, highlighting the robustness of our rule set in achieving definitive architectural recovery. Furthermore, if multiple structures exist in the previous layer, the incompatibility with rules in the current or any preceding layer will further narrow down the solutions, even when multiple ifmap parameters are considered. This makes it highly unlikely for the mechanism to recover multiple potential architectures. Even when there are minor changes between architectures, the probability of recovering the same structure is low due to the previous mentioned reasons. It is important to note that a minor change in one layer alters the ofmap and side-channel information, which cascades to affect the side-channel values of preceding layers, thereby recovering distinct CNN structures through the proposed method. For example, a minor change in one layer, such as altering the filter size in the second convolutional layer of AlexNet from a 5x5 to a 4x4, while maintaining all other parameters, leads to significant changes in the derived side-channel information, such as weight reads (from 614400 to 393216), psum reads (from 44603136 to 25489408) and writes (from 44789760 to 25690112), and \textit{event cycle} (from 27 to 29). Our method successfully adjusted to these changes to accurately recover the modified layer parameters, showing robustness over minor changes in structure. We have included this discussion in Section~\ref{subsec:applicability}.


%The slight possibility of encountering multiple solutions for a specific model and dataflow architecture combination is significantly outweighed by the risk this poses to model owners and users.

% \begin{itemize}
%     \item The mechanism use layer-by-layer structure extraction.
%     \item If we focus on a single layer extraction, Core of both algorithm is integer factorization to get initial potential result set and applying set of rules based on architectural hints and side channel info to converge the results to a single architecture.
%     \item Even though the paper does not provide formal validation of the mechanism that a particular side channel information and architectural hints converged the deduced to single layer structure. The experimental results demonstrates that for all 64 layers in all CNN models explored across 6 dataflow accelerators (384 combinations) converged to a single layer structure. 
%     \item This highlight the fact the set of rules in our mechanism are sufficient enough to converge the solutions.
%     \item Therefore, there it is evident that its highly unlikely for layer to consider multiple ifmap parameters ($X, Y, C$) from preceding layer to recover current layer.
%     \item Furthermore, if there are multiple structures in previous layer the incompatibility to adhere to rules in the current layer or any preceding layer would further converge the solutions even after multiple ifmaps are considered.
%     \item If there are minor changes between architecture the mechanism have a low chance of recovering the same architecture for the same two reasons. 
%     \item Furthermore, it is important to note that a smaller change in a one layer changes the ofmap of the layer and side channel information for that layer and have cascading effect on the preceding layer side channel values. For example, if we think a hypothetical scenario minor change to second convolution layer of alexnet by changing filter size (5x5 filter changed to 4x4), while keeping all the other parameters unchanged. This minor change to the layer change the wieghts reads (from 614400 to 393216), psum reads (from 44603136 to 25489408), psum writes (from 44789760 to 25690112) and event cycle (27 to 29). And we were able to successfully recover the exact layer parameters from this updated layer using our mechanism.
%     \item When thinking from a adversaries perspective, the minor possibility of having multiple solutions to specific model and dataflow architure combination is insignificant by this kind of recovery is put model owners at substantial risks.
% \end{itemize}



\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 11:} Table 1 is given too late.


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. We have moved the table closer to where it is discussed.


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 12:} There are many algorithms and it is not always easy to follow what algorithm authors discuss at what moment.


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. We have restructured the paper to move the algorithms as close as possible to its discussion.


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 13:} Most of the time, the number of filters ($K$) is greater than the number of PE arrays ($n$) of the accelerator architecture, then $n_a=n$. -> what happens when it is not like that?


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. The value of $n_a$ is calculated as $w[1]/i[1]$ (line 3 of Algorithm 3). This means that the number of active PE arrays ($n_a$) is determined by the ratio $w[1]/i[1]$, regardless of whether $K$ (the number of filters) is greater than $n$ (the number of PE arrays) or not. All the dataflow accelerators we have reviewed, the number of PE arrays ($n$) typically ranges from 10 to 20. Moreover, convolutional layers in models usually have more filters than this range. Therefore, in the majority of cases, $K$ is greater than $n$, and as a result, $w[1]/i[1]$ equals $n$. In other words, most convolutional layers will utilize all the PE arrays during the inference process, leading to $n_a = n$. However, if $K$ is not greater than $n$, the number of active PE arrays ($n_a$) will still be given by $w[1]/i[1]$. We modified relevant sentences in Section~\ref{subsec:recover_conv_ws} to resolve this confusion.


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 14:} gives the number of tiles -> what are tiles?


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. A tile is a subset of the input feature map or the output feature map that is processed as a unit. It can be thought of as a smaller "block" or "portion" of the overall feature map. The OS dataflow generates the output feature map as multiple tiles at a time if the number of PEs are smaller than the size of output feature map (ofmap). For example, consider ofmap is 8x8 and there are 4 PE arrays with 8 PEs per array. The ofmap is generated as two tiles (first tile covering first 4 rows of the ofmap and second covering the last four rows). We have provided the definition of `tile' in the relevant discussion found in Section~\ref{subsec:recover_conv_os}


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 15:} dataflow and underneath accelerator -> what does this mean?


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. We have corrected the typo and rephrased the sentence to: `FC layer parameters can be determined independent of the dataflow architecture by solely examining the total data reads and writes for the layer'.


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 16:} The authors consider average and max pooling. What about GAP?


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. In our study, we did not specifically consider Global Average Pooling (GAP) because the dataflow architectures under review do not typically incorporate GAP, and its operation is fundamentally simpler compared to average and max pooling. Unlike average and max pooling, which involve hyperparameters such as stride and filter size, GAP operates by computing the average of each feature map channel in the output feature map (ofmap). This results in a single average value per channel, effectively producing a vector of size $K$ (number of output channels) for an ofmap of dimensions $X' \times Y' \times K$. As GAP lacks configurable parameters beyond its basic function, the only information we can derive from side-channel analysis is the usage of GAP in a particular layer. This can be made by examining the side-channel data ($N_{pool}$) obtained from DRAM via the GB bus (\redcircleletter{c} in Figure \ref{fig:overview_of_accel}). If $N_{pool}$ corresponds exactly to the number of output channels ($K$), it indicates the use of GAP; otherwise, it does not. We have included this discussion in  Section~\ref{subsubsec:extractin_poool_layer}.


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 17:} The authors do not mention at all how to recover activation functions? I would assume this also to be important part of the architecture?


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. We acknowledge the importance of activation functions as integral components of a DNN's architecture. In our study, the state-of-the-art dataflow CNN inference accelerators we reviewed, such as those documented in \cite{chen2016eyeriss, chen2019eyeriss}, incorporate the Rectified Linear Unit (ReLU) as the sole activation function. This choice is based on empirical evidence suggesting that CNNs typically achieve better performance with ReLU in their hidden layers~\cite{agarap2018deep}. Consequently, our attack framework did not consider the explicit recovery of activation functions. Regarding the final layer, the type of activation function employed can often be inferred based on the specific task that the model addresses. For instance, multi-class classification tasks generally use a softmax activation function, whereas binary classification tasks might use a sigmoid function. It is important to note that these final layer activations (e.g. sigmoid, softmax) are usually executed outside the dataflow accelerator, on the host CPU~\cite{sze2017efficient}. However if future dataflow accelerators support a variety of activation functions, such as Leaky ReLU or Parametric ReLU, our proposed method to identify the activation function is to monitor which specific functional unit is activated during the processing of each layer. We have included this discussion in Section~\ref{subsubsec:identification_of_activation}.



% Thank you for the comment. We agree that activation function is a important part of a DNN model architecture. State of the art dataflow CNN inference accelerators we reviewed contained only a rectified linear unit (ReLU) module as the supported activation function~\cite{chen2016eyeriss,du2015shidiannao}. The main reason behind this is CNNs are known to perform better with ReLu activation in their hidden layers. Therefore, there was no need for our attack to explicit determination of the activation function. When we consider the output layer the activation function that is used can be determine using the problem that the model tries to solve. For example if its multi-class classification output layer will employ a softmax activation function and if its binary it will employ a sigmoid function. It's important to note that the output layer activation is done outside the accelerator in Host CPU. 

% But there can be a scenario where variations of ReLu such as Leaky ReLU and Parametric ReLU are supported by the future CNN dataflow accelerators. In case of multiple activation functions available in accelerator we propose the following method to recover the activation. Each of the activation functions will be implemented as separate functional units and we can simply check which functional unit is activated at each layer processing and determine which activation functions have been used in each layer. We have included this discussing into Section~\ref{sec:methodalogy}

% Upon reflection, we realize that our initial focus was primarily on structural elements such as input/output feature maps and weights, primarily due to [insert reason]. Activation functions, which play a crucial role in the non-linear processing capabilities of CNNs, were not addressed in our mechanism.

% To rectify this, we propose the following methods for future incorporation into our framework [provide brief overview of proposed methods]. We believe these enhancements will allow for a more comprehensive recovery of CNN architectures, including the vital non-linear components introduced by activation functions. As part of our ongoing and future work, we aim to validate these methods through [mention any planned experiments or analyses]. This will strengthen our approach and ensure a more complete architectural recovery.


% \begin{itemize}
%     \item two main reasons (1). the accelerators have fixed set of activation functions. Mostly one (2). Typically CNN uses ReLu or some 
%     \item Accelerators provide selected set of activation function units. Most accelerators provide Therefore
%     \item CNN typically use ReLu or derivation of ReLu.
%     \item In case of multiple activation functions available in accelerator we propose to recover the architecture using the proposed method and then iterate over the available 
%     \item we can simply check which functional unit is activated at each layer processing and determine which activation functions have been used in each layer.
% \end{itemize}

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 18:} and an in-house cycle-accurate simulator -> could you provide some details?


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. The cycle-accurate stonne simulator only supports WS dataflow. Therefore, we performed modifications on top of the stonne simulator to model OS dataflows. We have revised the sentence to accurately convey this information.


% \color{black}
% \vspace{0.1in}
% \noindent \textbf{Comment 19:} I find Table 2 difficult to read and interpret the results.


% \color{blue}
% \vspace{0.1in}
% \noindent \textbf{Response:} Thank you for the comment. 


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 19:} For example, the targeted event cycle in the second -> please explain in more detail.


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. As detailed in Section~\ref{subsec:recover_conv_ws}, the \textit{targeted event cycle}, denoted as $t_e$, is identified when $i[1] = i[t_e]$, meaning it is the cycle where the number of input reads matches those of the first cycle. The observed side channel value for \textit{targeted event cycle} of all convolutional layers in Alexnet is listed in fifth column of Table~\ref{tab:sc_ws_alexnet}, which is 27 for second convolutional layer. This is further illustrated in Figure~\ref{fig:example_ws_alex_conv2_graph}, where for the second convolutional layer, $t_e$ is pinpointed at cycle 27.


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 20:} I do not understand why the authors did not immediately present the algorithms in such a way to allow for relaxed assumptions from Section 5.5? And not there discuss how everything can be adapted and still work (without giving results).


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. The primary reason for initially presenting the algorithms with two specific assumptions was to simplify the explanation of our CNN architecture recovery mechanism. This makes it easier for readers to grasp the concepts without the introduction of complexity (additional variables). It also allows for clearer and concise visualization in timing diagrams (Figure~\ref{fig:example_ws_alex_conv2_graph} and ~\ref{fig:example_os_alex_conv1_graph}). Furthermore, these assumptions are not critical to our methodology for extracting the layer structure. While we refer to them as assumptions, it is technically feasible for certain accelerators to adhere to these assumptions. For instance, in a WS(4,4) accelerator, it is practical to have an input load bus of width 4, enabling the accelerator to save cycles on memory loading, or it could incorporate a pre-patching logic that virtually represent a non-bandwidth-limited bus from a width of one. Therefore, the current presentation of the algorithms enhances the readability of the paper and generalizability across different architectures.

% \begin{itemize}
%     \item The main reason for explaining the algorithms with two assumptions is to simplify the our CNN architecture recovery approach so that readers better understand it without introducing more variable to the algorithm and furthermore it is easy to visualize in timing diagrams. 
%     \item Furthermore, those two assumptions are not critical to the methodology of the layer structure extraction.
%     \item Eventhough we presented them as assumptions it is technically feasible for a particular accelerator to actually adhere to both assumptions. For example, a for a WS(4,4) accelerator it is  feasible to have a input load bus of width 4, so that the accelerator saves up cycles in memory loading or it can have a pre-patching logic that virtually no-bandwith limited bus from width o1 bus.
% \end{itemize}


% \begin{itemize}
%     \item avoid unnecessary complication to the algorithms and focus on core concepts used in algorithm for understanding.s
%     \item the core of the algorithm is 
%     \item As discussed earlier there are different variation of WS and OS dataflow accelerators with subtle differences. Our intuition was to show that the proposed attack can be can be done in any of the dataflow based accelerators. Therefore, we evaluate the attack on the simpler WS and OS models and then discuss the extension of the attack ..
% \end{itemize}


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 21:} can be extended to any WS accelerator with input forwarding as MAERI ~\cite{kwon2018maeri}. Our attack on OS dataflow can be extended to other OS architectures with input forwarding~\cite{du2015shidiannao,moons201714} to recover CNN models. -> at least discuss more (if not showing it).


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. The proposed attack can be extended to any WS accelerator with input forwarding, such as MAERI~\cite{kwon2018maeri}, by leveraging the hierarchical interconnects and input forwarding mechanisms to infer memory access patterns and extract CNN model parameters. The main difference between MAERI and the WS architecture in the paper lies in their reconfigurable interconnects, allowing dynamic adjustment of PE array size when processing each layer. This control message for reconfiguration can be snooped from the same bus (\redcircleletter{d} in Figure \ref{fig:overview_of_accel}) used in layer boundary identification (Section~\ref{subsec:identify_layer_boundary}). Once the PE size is determined through snooping, the proposed attack can be applied accordingly.
Both output stationary (OS) architectures, ShiDianNao~\cite{du2015shidiannao} and Envision~\cite{moons201714}, adhere to the OS architectures with input forwarding outlined in the paper, with subtle implementation differences. For example, Envision, rather than having dedicated input forwarding at each PE array, uses a FIFO buffer shared between PE arrays for input forwarding. Since this does not change the observed side-channel information (number of reads and writes) outside of the PE arrays, our attack can be extended to this architecture as well. These extensions are feasible because both WS and OS architectures share fundamental characteristics in data movement and reuse that were exploited in the attacks to recover model parameters and structures. We have included this discussion in Section~\ref{subsec:applicability}.


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 22:} It seems that the authors do not mention a number of related works. For instance:
\begin{itemize}
    \item \href{https://arxiv.org/abs/2312.07783}{https://arxiv.org/abs/2312.07783}~\cite{horvath2023barracuda}
    \item \href{https://arxiv.org/abs/2401.13575}{https://arxiv.org/abs/2401.13575}~\cite{horvath2024cnn}
    \item \href{https://link.springer.com/chapter/10.1007/978-3-030-81645-2_7}{https://link.springer.com/chapter/10.1007/978-3-030-81645-2-7}~\cite{chmielewski2021reverse}
\end{itemize}


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. We have included the suggested papers in the related work discussion (Section~\ref{subsec:related_work}).

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 23:} 

\textbf{Minor Comments:}
\begin{itemize}
    \item "Edge artificial intelligence (AI) has the benefit of overcoming edge-to-server communication bottlenecks, high availability without depending on the internet, real-time insights, and reduced storage." - Needs a reference.
    \item "Are preferred for inference at edge devices." - Needs a reference.
    \item "Multiple taxonomies [2]" - Should it be "multiple taxonomies" or "types in a taxonomy"?
    \item "ASIC-based accelerators are preferred in edge inference since they are energy efficient while providing adequate computational flexibility." - Needs a reference.
    \item Use "Section" consistently, not "section" or "the Section/section."
    \item "(line3) and" - Should be "line 3."
    \item "This needs an adversary needs to collect or actively" - Sentence appears incomplete or redundant. Clarification needed.
    \item "Most CNN accelerators use a separate low-bandwidth bus (d in Figure 4) to send these configurations." - Needs a reference.
    \item "Figure 4 (They" - "They" should be lowercase.
    \item "( // is" - Remove extra space.
    \item "Relationship stated in Equation 4 holds" - Should be "hold."
    \item "Architecture conducts" - Should be "conduct."
    \item "Then let’s look" - Avoid contractions; use "Let us look" instead.
    \item "( 2927232 =" - Remove extra space.
\end{itemize}


\color{blue}
\vspace{0.1in}
\noindent \textbf{Response:} Thank you for the suggested improvements. We have addressed them in the manuscript.  


\color{black}
\vspace{0.1in}
\subsection{REVIEWER 3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent \textbf{Comment 1:} I like the idea of bus snooping to obtain (hyper)parameters of a CNN. However, this is not a completely novel idea: it has been done by, e.g., Hu et al.~\cite{hu2020deepsniffer}. Therefore, I highly encourage reformulating the contributions of this paper to the field and better explore the related work.

\color{blue}

\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. We have reviewed the work presented in ~\cite{hu2020deepsniffer} and reformulated our first contribution to better explore the related work: `We adapt and refine the bus snooping-based threat model, originally applied to GPUs in ~\cite{hu2020deepsniffer}, to gather memory-based side-channel information from dataflow-based CNN inference accelerators.' This adjustment highlights our method's extension to new contexts and architectures.

\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 2:} Then just a small comment on the usage of superscript in the algorithms. It is quite confusing to see superscript being used, as this typically indicates exponential operations. Therefore I suggest using subscripts but with, e.g., a separating comma.


\color{blue}

\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your valuable input. We have replaced the superscript with subscript separating commas.


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 3:} As for the results, I miss the experimental part of the results. Currently, a simulator has been used to get the results. However, when using a real machine other difficulties will arise with capturing signals from the busses. Therefore I encourage you to spend more time in getting more realistic results instead of just the simulated ones.

\color{blue}

\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. We recognize the importance of validating our findings in a real-world setting and have taken significant steps to address this. We expanded our experiments to include real hardware implementations of the two weight stationary accelerator architectures (\textit{WS(4,4), and WS(12,4)}) detailed in Section~\ref{sec:experiments}. These architectures were implemented on the Alchitry Cu FPGA board, which utilizes the Lattice iCE40 HX FPGA supported by the open source tool chain IceStorm. The configuration parameters of the accelerator implementation in our experiments are outlined in Table~\ref{tab:com-acc-config}. 




\begin{table}[htp]
\centering
\caption{WS accelerator configuration parameters}
\vspace{-0.1in}
\label{tab:com-acc-config}
\resizebox{0.50\textwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
\textbf{Parameter} & \textbf{Value} \\ \hline
PE array dimensions: (m,n) & {[}(4,4), (12,4){]} \\ \hline
Precision (weights, ifmap, ofmap) & 8 bits \\ \hline
GB to PE arrays input bus width & $4 \times 8$ bits \\ \hline
GB to PE arrays weight bus width & $4 \times 8$ bits \\ \hline
Accumulator tree precision & 32 bits \\ \hline
Accumulated output bus width & $4 \times 32$ bits \\ \hline
Input forwading path width & 8 bits \\ \hline
Global buffer size & 256B \\ \hline
\end{tabular}%
}
\end{table}

Due to space limitations on the FPGA, we opted for a relatively small global buffer (GB). However, this constraint does not affect our ability to accurately recover side-channel information regarding the number of memory reads and writes from GB. We use a Python frontend, similar to the one used in STONNE~\cite{munoz2021stonne}, to emulate the host CPU. The UART (Universal Asynchronous Receiver/Transmitter) communication protocol is employed to facilitate serial communication between the Python frontend and the FPGA-implemented accelerator. This setup allows us to send control and data to the accelerator and receive snooped side-channel information from the accelerator. To facilitate the capture of memory-based side-channel information, particularly the number of memory reads and writes from the GB, we used snooping on the bus between the GB and the processing element array (\redcircleletter{a}
 in Figure \ref{fig:overview_of_accel}), as well as between the DRAM and GB (\redcircleletter{c}
 in Figure \ref{fig:overview_of_accel}). Snooping of buses was achieved by embedding two Hardware Trojans (HTs) into the RTL of the accelerator, analogous to the use of hardware performance counters in GPUs to emulate snooping, as discussed in previous studies~\cite{hu2020deepsniffer}. We conducted experiments using the CNN models initially employed in our simulations (Lenet, AlexNet, and VGGnet-16) plus YOLOv2~\cite{redmon2016you} which was introduced in this revision. Each model was subjected to 10 rounds of experiments to ensure robustness and repeatability of results. 
 
Our findings from these real-world experiments align with the results from cycle-accurate simulation, successfully recovering the exact architecture of all four CNN models every time, across all tested WS dataflow configurations. Furthermore, we want to emphasize that bus snooping, particularly through microprobing, has been extensively demonstrated in the literature~\cite{huang2002keeping,huang2014hmtt,blass2012tresor,shi2016layout,tajik2017power,wang2017probing} to accurately recover a variety of information from data buses with high precision, such as exact encryption keys. This technique has been effectively utilized in threat models for scenarios including the precise recovery of DNN architectures from GPUs. In our work, we focus on mechanism to extract CNN model architectures from dataflow-based accelerators, rather than revisiting the established methodologies of how to effectively implement bus snooping via microprobing. We have included details of these new experiments, results and experimental setup in Section~\ref{sec:experiments}.


% \begin{itemize}
%     \item To conduct more realistic experiments, we model three concrete weight-stationary accelerator architectures (\textit{WS}($4,4$), \textit{WS}($12,4$), and \textit{WS}($24,10$)) used in Section~\ref{sec:experiments} in FPGA.
%     \item For this we used Alchitry Cu that uses Lattice iCE40 HX FPGA.
%     \item In order to capture side channel information ( number of memory reads and writes from global buffer) needed for the proposed attack we snoop bus between global buffer (GB) and processing element array and bus between DRAM and GB.
%     \item To snooping we embed two HTs to RTL of the accelerator. Similarly in ~\cite{hu2020deepsniffer}  hardware performance counters of GPU has been used to emulate snooping.
%     \item We used three CNN models ( Lenet, AlexNet, and VGGnet-16) used in initial experiments in this experiment setup with additional YOLOv2~\cite{redmon2016you} introduced in this revision.
%     \item We conducted 10 rounds of experiments using 10 models of the same architecture. 
%     \item We were able to recover the exact models for all four CNN architecture each time across all three WS dataflow accelerator configurations.
%     \item Furthermore, we want to highlight Bus snooping is a low-cost, practical and well understood attack that has been widely demonstrated~\cite{huang2002keeping,huang2014hmtt,blass2012tresor} and utilized for several scenarios including recovering DNN architecture from GPUs~\cite{hu2020deepsniffer,hua2018reverse}. 
% \end{itemize}




% \begin{itemize}
%     \item Implement WS dataflow in a FPGA.
%     \item try layer by layer extraction extraction.
%     \item find similar papers using FPGA, what kind of FPGA they use?
% \end{itemize}


% \textit{We can also use a noise model to simulate actual messurements (since the messurements are counts +-5 threat model can be used), find similar papers do so.  \textcolor{red}{~\cite{hu2020deepsniffer} also have a noise model similar to what I thought.}}


% \textcolor{red}{We use the GPU performance counter [34]
% to emulate bus snooping for kernel execution latency, kernel
% write, and read access volume information collection~\cite{hu2020deepsniffer}}


\color{black}
\vspace{0.1in}
\noindent \textbf{Comment 4:} Also the way in which the results are presented does not tell me much. I would like to know more than just if the structure can be recovered (Table 2). For instance what the accuracy? Does this work for multiple different models of the same architecture and what does the accuracy become then?

\color{blue}

\vspace{0.1in}
\noindent \textbf{Response:} Thank you for your comment. We have conducted architecture recovery on multiple different models (10 iterations) for the same architecture using both simulator and FPGA implementations. Across the benchmark CNN models, and for both weight stationary (WS) and output stationary (OS) architectures, our deterministic method with same side channel information consistently converged to the actual architecture of the CNN for every iteration.
In response to Comment 3, we demonstrate the accurate recovery of memory read and write counts from FPGA and discuss the feasibility of high-precision recovery through microprobing. This accurate recovery of CNN architecture, facilitated by architectural hints from dataflow inference accelerators, highlights how layer-specific mapping and processing enhance the leakage of CNN architectures. We have modified Section~\ref{sec:experiments} to include these experiment details and results.



% \begin{itemize}
%     \item We have conducted architecture recovery of multiple different models (10) for the same architecture in both simulator and FPGA implementation. 
%     \item For the benchmark CNN models we used and across both WS and OS architectures. Our attack was able to converge to one CNN architecture which is equivalent to the actual architecture.
%     \item Since our approach of recovering architecture of CNN is a deterministic algorithm for the architecture recovery it will produce the same result with same side channel information. 
%     \item In recovering side channel information from FPGA and response to comment 3 we highlight the feasibility of high precision recovery of number memory reads and writes as side channel information.
%     \item This accurate recovery of CNN architecture with the help of architectural hints of the dataflow inference accelerators highlight the fact that layer-specific mapping and processing of DNN layers helps to leak CNN architectures better. 
% \end{itemize}


% \begin{itemize}
%     \item Our attack methodology does not provide any randomness, the only way the recovery of multiple models of the same architecture differed is by the measurement errors from the side-channel. 
%     \item This highlight the fact that recovering exact CNN model architectures from datflow based architures in with architural hints 
%     \item mapping of the dataflow is tuned to the architecture.
% \end{itemize}

